VBSCan Mid-Term Scientific Meeting

This document summarises the talks and discussions happened during the VBSCan Mid-Term Scientific Meeting workshop. The VBSCan COST action is dedicated to the coordinated study of vector boson scattering (VBS) from the phenomenological and experimental point of view, for the best exploitation of the data that will be delivered by existing and future particle colliders.

==> FrontBackMaterial/SR_Abstract.tex <==
\begin{center} 
 {\bf Abstract}
\end{center}
\vspace{0.5cm}
%
  This document summarizes the talks and discussions happened during the VBSCan Split17 workshop,
  the first general meeting of the VBSCan COST Action network,
  aiming at a consistent and coordinated study of vector-boson scattering
  from the phenomenological and experimental point of view, 
  for the best exploitation of the data that will be delivered by the LHC future operations.





==> FrontBackMaterial/SR_Conveners.tex <==
\leftline{\bf Conveners}
\begin{flushleft}
\noindent \emph{WG1: Theoretical understanding:}
         M.~Pellen, M.~Zaro
\vspace{0.1cm}

\noindent \emph{WG2: Analysis techniques:} 	
         M.~Slawinska, R.~Covarelli
\vspace{0.1cm}

\noindent \emph{WG3: Experimental techniques:} 	
         S.~Duric, L.~S.~Bruni
\vspace{0.1cm}

\noindent \emph{WG4: Knowledge exchange and cross activities:}
	 K.~Lohwasser and I.~Puljak
\vspace{0.1cm}

\noindent \emph{WG5: Inclusiveness policies:}
	 C.~Petridou

\end{flushleft}

\endinput


==> FrontBackMaterial/SR_Title_Backside.tex <==
\null
\vfill


\endinput


==> SR_NewCommands.tex <==
%\newcommand{\Pl}{\ell}
\newcommand{\fb}{{\ensuremath\unskip\,\text{fb}}\xspace}
% % new commands for cross referencing
\def\reffi#1{\mbox{Figure~\ref{#1}}}
\def\reffis#1{\mbox{Figures~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}


\def\eq#1{{eq.~(\ref{#1})}}
\def\eqs#1#2{{eqs.~(\ref{#1})--(\ref{#2})}}
\def\fig#1{{figure~(\ref{#1})}}
\def\sec#1{{section~(\ref{#1})}}
\def\figs#1#2{{figures~(\ref{#1})--(\ref{#2})}}
\def\tab#1{{table~(\ref{#1})}}
\def\tabs#1#2{{tables~(\ref{#1})--(\ref{#2})}}
\def\app#1{{appendix~(\ref{#1})}}

%\newcommand{\ri}{\mathrm i}

%\newcommand{\ie}{\emph{i.e.}\ }

\def\be{\begin{equation}}
\def\ee{\end{equation}}
\providecommand{\tabularnewline}{\\}
                                    
%\newcommand{\Mt}{\ensuremath{m_\Pt}\xspace}
%\newcommand{\MH}{\ensuremath{M_\PH}\xspace}
\newcommand{\MWOS}{\ensuremath{M_\PW^\text{OS}}\xspace}
%\newcommand{\MW}{\ensuremath{M_\PW}\xspace}
\newcommand{\MZOS}{\ensuremath{M_\PZ^\text{OS}}\xspace}
%\newcommand{\MZ}{\ensuremath{M_\PZ}\xspace}
%\newcommand{\Mb}{\ensuremath{m_\Pb}\xspace}
\newcommand{\Gt}{\ensuremath{\Gamma_\Pt}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_\PH}\xspace}
\newcommand{\GZ}{\ensuremath{\Gamma_\PZ}\xspace}
\newcommand{\GZOS}{\ensuremath{\Gamma_\PZ^\text{OS}}\xspace}
\newcommand{\GW}{\ensuremath{\Gamma_\PW}\xspace}
\newcommand{\GWOS}{\ensuremath{\Gamma_\PW^\text{OS}}\xspace}

\newcommand{\MVOS}{\ensuremath{M_V^\text{OS}}\xspace}%
\newcommand{\GVOS}{\ensuremath{\Gamma_V^\text{OS}}\xspace}%

\newcommand{\GeV}{\ensuremath{\,\text{GeV}}\xspace}
\newcommand{\TeV}{\ensuremath{\,\text{TeV}}\xspace}

\newcommand{\alphas}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}{\left(#1\right)}}\xspace}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\deltar}{\ensuremath{\Delta R}\xspace}

\newcommand{\GF}{\ensuremath{G_\mu}}

\newcommand{\pt}{\ensuremath{p_\text{T}}\xspace}
\newcommand{\ptsub}[1]{\ensuremath{p_{\text{T},#1}}\xspace}

\newcommand{\et}{\ensuremath{E_\text{T}}\xspace}
\newcommand{\etsub}[1]{\ensuremath{E_{\text{T},#1}}\xspace}

\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}

\newcommand{\fullProcess  }{\ensuremath{\Pp\Pp\to\Pe^+\nu_\Pe \mu^-\bar{\nu}_\mu\Pb\bar{\Pb}}\xspace}
\newcommand{\ggProcess    }{\ensuremath{\Pg\Pg\to\Pe^+\nu_\Pe \mu^-\bar{\nu}_\mu\Pb\bar{\Pb}}\xspace}
\newcommand{\qqbProcess    }{\ensuremath{q\bar{q}\to\Pe^+\nu_\Pe \mu^-\bar{\nu}_\mu\Pb\bar{\Pb}}\xspace}

\newcommand{\recola}{{\sc Recola}\xspace}
\newcommand{\mocanlo}{{\sc MoCaNLO}\xspace}
\newcommand{\collier}{{\sc Collier}\xspace}
\newcommand{\madgraph}{{\sc\small MadGraph5\_aMC@NLO}\xspace}
\newcommand{\rT}{{\mathrm{T}}}
% \def\abs#1{{\color{red}#1}}
% \def\absq#1{{\color{green}#1}}
\newcolumntype{.}{D{.}{.}{-1}}
\newcolumntype{d}[1]{D{.}{.}{#1}}

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\lsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle <}{\sim}$}\;}
\newcommand{\gsim}
{\;\raisebox{-.3em}{$\stackrel{\displaystyle >}{\sim}$}\;}
\def\asymp#1{\;\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}\;}

\newlength{\width}
\newlength{\height}
\newcommand{\brabar}[1]{%
    \settoheight{\height}{\ensuremath{#1}}%
    \settowidth{\width}{\ensuremath{#1}}%
    \makebox[0pt][l]{\ensuremath{#1}}%
    \raisebox{1.26ex}{\scalebox{.3}{\textbf{(}}}%
    \rule[1.41\height]{0.7\width}{0.35pt}%
    \raisebox{1.26ex}{\scalebox{.3}{\textbf{)}}}%
}


% modifications for drafts for drafts
\newcommand{\mpar}[1]{{\marginpar{\hbadness10000%
                      \sloppy\hfuzz10pt\boldmath\bf\textcolor{red}{#1}}}%
                      \typeout{marginpar: #1}\ignorespaces}
\marginparwidth 1.2cm
\marginparsep 0.2cm
\def\draftdate{\relax}
\def\mda{\relax}
\def\mua{\relax}
\def\mla{\relax}
\def\draft{
\def\thtystars{******************************}
\def\sixtystars{\thtystars\thtystars}
\typeout{}
\typeout{\sixtystars**}
\typeout{* Draft mode!
         For final version remove \protect\draft\space in source file *}
\typeout{\sixtystars**}
\typeout{}
\def\draftdate{\today}
\def\mua{\marginpar[\boldmath\hfil$\uparrow$]%
                   {\boldmath$\uparrow$\hfil}\color{black}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\mda{\color{red}\marginpar[\boldmath\hfil$\downarrow$]%
                   {\boldmath$\downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\mla{\marginpar[\boldmath\hfil$\rightarrow$]%
                   {\boldmath$\leftarrow $\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\def\Mua{\marginpar[\boldmath\hfil$\Uparrow$]%
                   {\boldmath$\Uparrow$\hfil}\color{black}%
                    \typeout{marginpar: $\uparrow$}\ignorespaces}
\def\Mda{\color{red}\marginpar[\boldmath\hfil$\Downarrow$]%
                   {\boldmath$\Downarrow$\hfil}%
                    \typeout{marginpar: $\downarrow$}\ignorespaces}
\def\Mla{\marginpar[\boldmath\hfil\textcolor{red}{$\Rightarrow$}]%
                   {\boldmath\textcolor{red}{$\Leftarrow $}\hfil}%
                    \typeout{marginpar: $\leftrightarrow$}\ignorespaces}
\overfullrule 5pt
\oddsidemargin 15mm
\marginparwidth 29mm
}

% switch on draft mode
%\draft



==> authors.tex <==
%\author[HEI]{Anders, Christoph Falk}    
\author[CER]{Baglio, Julien}
\author[TOI]{Ballestrero, Alessandro}
%\author[MAI]{Balz, Johannes}            
\author[TOR]{Bellan, Riccardo}
%\author[DES]{Bernhard Meyer, Andreas}
%\author[WUR]{Biedermann, Benedikt}
\author[TUD]{Bittrich, Carsten}
\author[DES]{Bra\ss{}, Simon}
\author[HEI]{Brivio, Ilaria}            
%\author[NIK]{Bruni, Lucrezia Stella}    
\author[CSE]{Buarque Franzosi, Diogo}
%\author[UCL]{Butterworth, Jonathan}
%\author[LPT]{Cacciari, Matteo}
%\author[FIR]{Cardini, Andrea}           
%\author[MIT]{Gomez-Ceballos, Guillelmo}
\author[LLR]{Charlot, Claude}     
%\author[FIR]{Ciulli, Vitaliano}      
\author[TOR]{Covarelli, Roberto}
\author[UOV]{Cuevas, Javier}
%\author[CP3]{Degrande, C\'eline}
\author[FIRI]{L. Delgado, Rafael}
%\author[WUR]{Denner, Ansgar}
%\author[FRE]{Dittmaier, Stefan}
%\author[LAP]{Di Ciaccio, Lucia}
%\author[WIN,KAN]{Duric, Senka}
%\author[WAW]{Farrington, Sinead}
%\author[NIK]{Ferrari, Pamela}           
%\author[CER]{Ferreira Silva, Pedro}
%\author[TOR]{Finco, Linda}
\author[LIS]{Gallinaro, Michele}
%\author[SPL]{Giljanovi\'c, Duje}             
%\author[DUR]{Glover, Nigel}
\author[DUR]{Gomez-Ambrosio, Raquel}    
%\author[FRE]{Gonella, Giulia}           
\author[MIB]{Govoni, Pietro}            
%\author[LAP]{Goy, Corinne}
%\author[CEA]{Gras, Philippe}            
%\author[DES]{Grojean, Christophe}
%\author[WEI]{Gross, Eilam}
\author[PBM]{Grossi, Michele}
%\author[DUB]{Grunewald, Martin}
%\author[CER]{Helary, Louis}
%\author[TUD]{Herrmann, Tim}
%\author[WIN]{Herndon, Matt}
%\author[HAM]{Hinzmann, Andreas}         
%\author[TUD]{Iltzsche, Franziska}
%\author[TUB]{J\"ager, Barbara}
%\author[ANT]{Janssen, Xavier}           
%\author[DES]{Jung, Hannes}
\author[ROX]{Karlberg, Alexander}       
\author[COU]{Kayis Topaksu, Aysel}
%\author[PRA]{Kepka, Oldrich}
\author[LJUMP]{Kersevan, Borut}
\author[SIG]{Kilian, Wolfgang}
\author[KIT]{Kirchgae\ss{}er, Patrick}
%\author[MIT]{Klute, Markus}
%\author[TUD]{Kobel, Michael}
%\author[LAP]{Koletsou, Iro}
%\author[THE]{Kordas, Kostas}            
%\author[UWAR,GES]{Koz{\'o}w, Pawe{\l}}
%\author[NCU]{Kuo, Chia-Ming}
%\author[HEL]{Lampen, Tapio}
%\author[ANT]{Lauwers, Jasper Gerard E.} 
%\author[SPL]{Lelas, Damir}              
%\author[FIR]{Lenzi, Piergiulio}
%\author[PEK]{Li, Qiang}
%\author[DUR]{Lindert, Jonas}
%\author[DES]{Lipka, Katerina}
\author[SHE]{Lohwasser, Kristin}        
%\author[WIN]{Long, Kenneth}
\author[LAP]{Lorenzo Martinez, Narei}   
\author[TOR]{Maina, Ezio}               
%\author[CP3]{Maltoni, Fabio}
%\author[TUD]{Manjarres, Joany}          
%\author[TOI]{Mariotti, Chiara}
\author[CP3]{Mattelaer, Olivier}
\author[ELU]{Mehta, Ankita}
%\author[SHE]{Mildner, Hannes}
\author[BEL]{Milenovic, Predrag}
%\author[KIT]{Mozer, Matthias Ulrich}    
%\author[CER]{Mulders, Martijn}
\author[ICISE]{Ninh, Le Duc}
\author[LJU]{Novak, Jakob}                 
%\author[MIB]{Oleari, Carlo}
\author[LFR]{Ortona, Giacomo}
\author[PRU]{\"Ozdemir, Kadri}
%\author[MOX]{Paganoni, Anna}
\author[EDI]{Papaefstathiou, Andreas}
\author[ELU]{P\'asztor, Gabriella}
\author[CAM]{Pellen, Mathieu}           
\author[TOR,WUR]{Pelliccioli, Giovanni}
\author[THE]{Petridou, Chara}       
%\author[LLR]{Pigard, Philipp}           
\author[UVA,ESI]{Pl\"atzer, Simon}
%\author[HEI]{Plehn, Tilman}
%\author[BNL]{Pleier, Marc-Andre}
%\author[PAI]{Polesello, Giacomo}
%\author[DES]{Potamianos, Karolos}
%\author[MAN]{Price, Darren}             
\author[SPL]{Puljak, Ivica}             
%\author[KIT]{Rauch, Michael}            
\author[PAV]{Rebuzzi, Daniela}          
\author[DES]{Reuter, J\"urgen}
%\author[CER]{Riva, Francesco}
%\author[DES]{Rothe, Vincent}
\author[CP3]{Ruiz, Richard}
%\author[SIE]{Russo, Lorenzo}            
%\author[CER]{Salam, Gavin}
%\author[LLR]{Salerno, Roberto}
\author[THE]{Sampsonidou, Despoina}     
%\author[MOX]{Sangalli, Laura}
%\author[LBN]{Shapiro, Marjorie}
\author[LAP]{Sauvan, Emmanuel}
%\author[FRE]{Schumacher, Markus}
%\author[FRE]{Schwan, Christopher}       
%\author[KIT]{Sekulla, Marco}
%\author[CER]{Selvaggi, Michele}
\author[MIN,OIN]{Shil, Sujay}
%\author[TUD]{Siegert, Frank}
\author[PAS]{Slawinska, Magdalena}      
%\author[NIK]{Snoek, Hella}
\author[SHE]{Sommer, Philip}            
%\author[DUR]{Spannowsky, Michael}
%\author[LON]{Span\`o, Francesco}
%\author[DES]{Stienemeier, Pascal} 
%\author[KTH]{Strandberg, Jonas}         
\author[WAR]{Szleper, Micha\l{}}    
%\author[UER]{Sznajder, Andre}       
%\author[FNA]{Tkaczyk, Swavek}
\author[TUD]{Todt, Stefanie}
%\author[NIE]{Trott, Michael}
%\author[THE]{Tzamarias, Spyros}         
\author[CER,MIC]{Valsecchi, Davide}
%\author[NIK]{Van Eijk, Bob}
\author[LFR]{Varouchas, Dimitris}
%\author[MIC]{Vicini, Alessandro}
\author[CP3]{Vischia, Pietro}
%\author[HEL]{Voutilainen, Mikko}        
%\author[CER]{Vryonidou, Eleni}
%\author[CER]{Zanderighi, Giulia}
\author[NIK,MIB]{Zaro, Marco}               
%\author[KIT]{Zeppenfeld, Dieter}


%\affil[ANT]{University of Antwerp (BE)}
%\affil[BNL]{Physics Department, Brookhaven National Laboratory, Upton NY (US)}
\affil[BEL]{Faculty of Physics, University of Belgrade (RS)}
\affil[CAM]{University of Cambridge (UK)}
%\affil[CEA]{CEA/Saclay - IRFU (FR)}
\affil[COU]{Cukurova University, Science and Art Faculty, Physics Department,  Adana, Turkey}
%\affil[CNR]{Centre National de la Recherche Scientifique (FR)}
\affil[CER]{CERN (CH)}
%\affil[CP3]{Centre for Cosmology, Particle Physics and Phenomenology Universit\'e{} catholique de Louvain (BE)}
\affil[CP3]{Centre for Cosmology, Particle Physics and Phenomenology Universit\'e{} catholique de Louvain, B-1348 Louvain-la-Neuve (BE)}
\affil[CSE]{Chalmers University of Technology, G\"oteborg (SE)}
\affil[DES]{Deutsches Elektronen-Synchrotron, Hamburg (DE)}
%\affil[DET]{DESY Theory Group, Notkestr. 85, 22607 Hamburg (DE)}
%\affil[DUB]{University College Dublin (IE)}
%\affil[DUB]{University College Dublin, Belfield 4, Dublin (IE)}
%\affil[DUR]{Institute for Particle Physics Phenomenology, Department of Physics, University of Durham (UK)}
\affil[DUR]{Institute for Particle Physics Phenomenology, Department of Physics, University of Durham, Durham DH1 3LE (UK)}
\affil[EDI]{Higgs Centre for Theoretical Physics, University of Edinburgh (UK)}
%\affil[EKU]{Institute for Theoretical Physics, Eberhard Karls University T\"ubingen, T\"ubingen (DE)}
\affil[ELU]{MTA-ELTE Lend\"ulet CMS Particle and Nuclear Physics Group, E\"otv\"os Lor\'and University, Budapest (HU)}
\affil[ESI]{Erwin Schr\"odinger International Institute for Mathematical Physics (ESI), Boltzmanngasse 9, A-1090 Vienna, Austria}
%\affil[ETH]{Universit\"at Z\"urich (CH)}
%\affil[FNA]{Fermi National Accelerator Laboratory, Batavia (US)}
%\affil[FIR]{University and INFN, Firenze (IT)}
\affil[FIRI]{INFN, Firenze (IT)}
%\affil[FRE]{Albert-Ludwigs-Universit\"at Freiburg (DE)}
%\affil[GES]{Universidad de Granada, Granda (ES)}
%\affil[HAM]{University of Hamburg (DE)}
\affil[HEI]{Ruprecht-Karls-Universit\"at Heidelberg (DE)}
%\affil[HEL]{University of Helsinki and HIP (FI)}
\affil[ICISE]{Institute For Interdisciplinary Research in Science and Education, ICISE, Quy Nhon, (VN)}
%\affil[KAN]{Kansas State University (US)}
\affil[KIT]{KIT - Karlsruhe Institute of Technology (DE)}
%\affil[KTH]{KTH Royal Institute of Technology (SE)}
\affil[LAP]{LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS/IN2P3, Annecy (FR)}
%\affil[LBN]{Lawrence Berkeley National Laboratory and University of California, Berkeley (USA)}
\affil[LFR]{LAL, Universit\'e Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, Orsay (FR)}
\affil[LIS]{LIP Lisbon (PT)}
\affil[LJU]{Department of Experimental Particle Physics, Jo\v{z}ef Stefan Institute and Department of Physics, University of Ljubljana (SI)}
\affil[LJUMP]{Faculty of Mathematics and Physics, University of Ljubljana (SI)}
\affil[LLR]{LLR, \'Ecole Polytechnique, CNRS/IN2P3, Universit\'e Paris-Saclay (FR)}
%\affil[LPT]{LPTHE Jussieu, Paris (FR)}
%\affil[LPT]{Sorbonne Universit\'es, UPMC Univ. Paris 06, UMR 7589, LPTHE, F-75005, Paris, France \emp{and} CNRS, UMR 7589, LPTHE, F-75005, Paris (FR)}
%\affil[LON]{Royal Holloway University of London (UK)}
%\affil[LPT]{Sorbonne Universit\'es and CNRS, LPTHE, Paris (FR)}
%\affil[LPT]{Sorbonne Universit\'es, UPMC Univ. Paris 06, UMR 7589, LPTHE, F-75005, Paris, France \textit{and} CNRS, UMR 7589, LPTHE, F-75005, Paris (FR)}
%\affil[MAI]{Johannes-Gutenberg-Universit\"at Mainz (DE)}
%\affil[MAN]{University of Manchester (GB)}
\affil[MIB]{INFN, Sezione di Milano, Via Celoria 16, 20133 Milano, (IT)}
\affil[MIB]{University and INFN, Milano-Bicocca (IT)}
\affil[MIC]{Universit\`a degli Studi di Milano (IT)}
\affil[MIN]{Homi Bhabha National Institute, Training School Complex, Anushakti Nagar, Mumbai (IN)}
%\affil[MIT]{Massachusetts Institute of Technology, Cambridge (US)}
%\affil[MOX]{MOX - Department of Mathematics, Politecnico di Milano (IT)}
%\affil[NCU]{National Central University, Chung-Li (TW)}
%\affil[NIE]{Niels Bohr International Academy and Discovery Center, Niels Bohr Institute, Copenhagen University (DK)}
%\affil[NIE]{Niels Bohr International Academy and Discovery Center, Niels Bohr Institute, Copenhagen University, Blegdamsvej 17, 2100 Copenhagen (DK)}
%\affil[NIE]{Niels Bohr Institute (DK)}
\affil[NIK]{Nikhef National institute for subatomic physics (NL)}
\affil[OIN]{Institute of Physics, Sachivalaya Marg, Bhubaneswar, Odisha (IN)}
\affil[ROX]{Rudolf Peierls Centre for Theoretical Physics, University of Oxford, Clarendon Laboratory, Parks Road, Oxford OX1 3PU (UK)}
\affil[PAS]{Polish Academy of Sciences (PL)}
\affil[PAV]{Universit\`a di Pavia e INFN, Sezione di Pavia (IT)}
%\affil[PAI]{INFN Pavia (IT)}
\affil[PBM]{University of Pavia and IBM Italy (IT)}
%\affil[PEK]{School of Physics and State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing (CN)}
%\affil[PRA]{Institute of Physics, Academy of Sciences of the Czech Republic, Praha (CZ)}
\affil[PRU]{P\^ir\^is Reis University, Engineering Faculty, Istanbul (TR)}
\affil[SHE]{University of Sheffield (GB)}
%\affil[SIE]{University of Siena and INFN Firenze (IT)}
\affil[SIG]{University of Siegen (DE)}
\affil[SPL]{University of Split, FESB (HR)}
\affil[THE]{Aristotle University of Thessalon\'iki (GR)}
\affil[TOI]{INFN Torino (IT)}
\affil[TOR]{University and INFN Torino (IT)}
%\affil[TUB]{University of T\"ubingen (DE)}
\affil[TUD]{Technische Universitaet Dresden (DE)}
%\affil[UCL]{Department of Physics and Astronomy, University College London (UK)}
%\affil[UCL]{Department of Physics and Astronomy, University College London, London (UK)}
%\affil[UER]{University of the State of Rio de Janeiro (BR)}
\affil[UOV]{University of Oviedo (SP)}
%\affil[UHH]{University of Hamburg, Hamburg (DE)}
\affil[UVA]{Fakult\"at Physik, University of Vienna, Vienna (AT)}
%\affil[UWAR]{University of Warsaw, Warsaw (PL)}
%\affil[WEI]{Weizmann Institute of Science (IL)}
\affil[WAR]{National Center for Nuclear Research, Warsaw (PL)}
%\affil[WAW]{Department of Physics, University of Warwick, Coventry (UK)}
%\affil[WIN]{University of Wisconsin-Madison (US)}
\affil[WUR]{University of W\"urzburg (DE)}


% nation codes: http://www.unece.org/cefact/locode/service/location



